Sensor Equivariance by LiDAR Projection Images

In this work, we propose an extension of conventional image data by an additional channel in which the associated projection properties are encoded. This addresses the issue of sensor-dependent object representation in projection-based sensors, such as LiDAR, which can lead to distorted physical and geometric properties due to variations in sensor resolution and field of view. To that end, we propose an architecture for processing this data in an instance segmentation framework. We focus specifically on LiDAR as a key sensor modality for machine vision tasks and highly automated driving (HAD). Through an experimental setup in a controlled synthetic environment, we identify a bias on sensor resolution and field of view and demonstrate that our proposed method can reduce said bias for the task of LiDAR instance segmentation. Furthermore, we define our method such that it can be applied to other projection-based sensors, such as cameras. To promote transparency, we make our code and dataset publicly available. This method shows the potential to improve performance and robustness in various machine vision tasks that utilize projection-based sensors.

==> bibliography.tex <==
\begin{thebibliography}{00}

\bibitem{xung}Hetzel, M. \& Reichert, H. Smart infrastructure: A research junction. {\em IEEE International Smart Cities Conference (ISC2)}. pp. 1–4 (2021)

\bibitem{decoint}Bieshaar, M. \& Reitberger, G. Detecting Intentions of Vulnerable Road Users Based on Collective Intelligence. {\em CoRR}. abs/1809.03916 (2018)


\bibitem{reitberger}Reitberger, G. \& Zernetsch, S. Cooperative Tracking of Cyclists Based on Smart Devices and Infrastructure. {\em 2018 21st International Conference On Intelligent Transportation Systems (ITSC)}. pp. 436-443 (2018)


\bibitem{continental}AG, C. Continental Launches Smart City Mobility and Transportation Hub for Safer and Smarter Cities. (https://www.continental.com/en-us/press-/press-releases/smart-city-mobility-205048) (2018)


\bibitem{eilbrecht}Eilbrecht, J. \& Bieshaar, M. Model-predictive planning for autonomous vehicles anticipating intentions of vulnerable road users by artificial neural networks. {\em 2017 IEEE Symposium Series On Computational Intelligence, SSCI 2017, Honolulu, HI, USA, November 27 - Dec. 1, 2017}. pp. 1-8 (2017)


\bibitem{koper}Goldhammer, M. \& Stiegel, E. Cooperative multi sensor network for traffic safety applications at intersections. {\em 2012 15th International IEEE Conference On Intelligent Transportation Systems}. pp. 1178-1183 (2012)


\bibitem{koper_data}Strigel, E. \& Meissner, D. The Ko-PER intersection laserscanner and video dataset. {\em 17th International IEEE Conference On Intelligent Transportation Systems (ITSC)}. pp. 1900-1901 (2014)


\bibitem{zernensch}Zernetsch, S. \& Reichert, H. Trajectory Forecasts with Uncertainties of Vulnerable Road Users by Means of Neural Networks. {\em 2019 IEEE Intelligent Vehicles Symposium (IV)}. pp. 810-815 (2019)


\bibitem{kress}Kress, V. \& Jung, J. Human Pose Estimation in Real Traffic Scenes. {\em 2018 IEEE Symposium Series On Computational Intelligence (SSCI)}. pp. 518-523 (2018)


\bibitem{bieshaar}Bieshaar, M. \& Zernetsch, S. Cooperative Starting Movement Detection of Cyclists Using Convolutional Neural Networks and a Boosted Stacking Ensemble. {\em CoRR}. abs/1803.03487 (2018)

\bibitem{dlr}DLR Institute of Transportation Systems AIM Research Intersection: Instrument for traffic detection and behavior assessment for a complex urban intersection. {\em Journal Of Large-scale Research Facilities}. Volume 2 pp. A65 (2016)


\bibitem{ulm}Ulm University. Pilotanalage für vernetztes Fahren. (https://www.uni-ulm.de/in/mrm/forschung/infrastruktur/pilotanlage-fuer-vernetztes-fahren) (2019)


\bibitem{survey}Shirazi, M. \& Morris, B. Looking at Intersections: A Survey of Intersection Monitoring, Behavior and Safety Analysis of Recent Studies. {\em IEEE Transactions On Intelligent Transportation Systems}. pp. 1-21 (2016,8)


\bibitem{highD}Krajewski, R. \& Bock, J. The highD Dataset: A Drone Dataset of Naturalistic Vehicle Trajectories on German Highways for Validation of Highly Automated Driving Systems. {\em 2018 21st International Conference On Intelligent Transportation Systems (ITSC)}. pp. 2118-2125 (2018)


\bibitem{inD}Bock, J. \& Krajewski, R. The inD Dataset: A Drone Dataset of Naturalistic Road User Trajectories at German Intersections. {\em 2020 IEEE Intelligent Vehicles Symposium (IV)}. pp. 1929-1934 (2020)


\bibitem{rounD}Krajewski, R. \& Moers, T. The rounD Dataset: A Drone Dataset of Road User Trajectories at Roundabouts in Germany. {\em 2020 IEEE 23rd International Conference On Intelligent Transportation Systems (ITSC)}. pp. 1-6 (2020)


\bibitem{nuscenes}Caesar, H. \& Bankiti, V. nuScenes: A multimodal dataset for autonomous driving. {\em ArXiv Preprint ArXiv:1903.11027}. (2019)


\bibitem{waymo_prediction}Sun, P. \& Kretzschmar, H. Scalability in Perception for Autonomous Driving: Waymo Open Dataset. {\em Proceedings Of The IEEE/CVF Conference On Computer Vision And Pattern Recognition (CVPR)}. (2020,6)


\bibitem{waymo_motion}Ettinger, S. \& Cheng, S. Large Scale Interactive Motion Forecasting for Autonomous Driving: The Waymo Open Motion Dataset. {\em Proceedings Of The IEEE/CVF International Conference On Computer Vision (ICCV)}. pp. 9710-9719 (2021,10)


\bibitem{pie}Rasouli, A. \& Kotseruba, I. PIE: A Large-Scale Dataset and Models for Pedestrian Intention Estimation and Trajectory Prediction. {\em International Conference On Computer Vision (ICCV)}. (2019)


\bibitem{eth}Pellegrini, S. \& Ess, A. You'll never walk alone: Modeling social behavior for multi-target tracking. {\em 2009 IEEE 12th International Conference On Computer Vision}. pp. 261-268 (2009)


\bibitem{ucy}Lerner, A. \& Chrysanthou, Y. Crowds by example. {\em Computer Graphics Forum}. pp. 655-664 (2007)


\bibitem{ssd}Robicquet, A. \& Sadeghian, A. Learning social etiquette: Human trajectory understanding in crowded scenes. {\em European Conference On Computer Vision}. pp. 549-565 (2016)


\bibitem{gc}Yi, S. \& Li, H. Understanding pedestrian behaviors from stationary crowd groups. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 3488-3496 (2015)


\bibitem{decoint_dataset}Zernetsch, S. VRU Trajectory Dataset. , https://www.th-ab.de/vru-trajectory-dataset (2020)

\bibitem{nelder_mead}Nelder, J. \& Mead, R. A Simplex Method for Function Minimization. {\em The Computer Journal}. \textbf{7}, 308-313 (1965,1)


\bibitem{arun_1987}Arun, K. \& Huang, T. Least-Squares Fitting of Two 3-D Point Sets. {\em IEEE Transactions On Pattern Analysis And Machine Intelligence}. PAMI-9, 698-700 (1987)


\bibitem{bar_shalom_2001}Bar-Shalom, Y. \& Li, X. Estimation with Applications to Tracking and Navigation: Theory Algorithms and Software. (John Wiley,2001)


\bibitem{imm_blair_shalom}Blair, W. \& Bar-Shalom, T. Tracking maneuvering targets with multiple sensors: does more data always mean better estimates?. {\em IEEE Transactions On Aerospace And Electronic Systems}. \textbf{32}, 450-456 (1996)


\bibitem{imm_genovese}Genovese, A. The interacting multiple model algorithm for accurate state estimation of maneuvering targets. {\em Johns Hopkins APL Technical Digest (Applied Physics Laboratory)}. Volume 22 pp. 614-623 (2001,10)


\bibitem{imm_diff_models_states}Yuan, T. \& Bar-Shalom, Y. A Multiple IMM Estimation Approach with Unbiased Mixing for Thrusting Projectiles. {\em IEEE Transactions On Aerospace And Electronic Systems}. Volume 48, 3250-3267 (2012)


\bibitem{bernardin_2008}Bernardin, K. \& Stiefelhagen, R. Evaluating Multiple Object Tracking Performance: The CLEAR MOT Metrics. {\em EURASIP Journal On Image And Video Processing}. 2008, 246-309 (2008)


\bibitem{pitre_2005}Ryan, R. \& Vesselin, P. A comparative study of multiple-model algorithms for maneuvering target tracking. {\em Signal Processing, Sensor Fusion, And Target Recognition XIV}. pp. 549 - 560 (2005), https://doi.org/10.1117/12.609681


\bibitem{hartley_2004}Hartley, R. \& Zisserman, A. Multiple View Geometry in Computer Vision. (Cambridge University Press,2004)


\bibitem{openCV3_kaehler}Kaehler, A. \& Bradski, G. Learning OpenCV 3: Computer Vision in C++ with the OpenCV Library. (O'Reilly Media, Inc.,2016)


\bibitem{kitti_2012}Geiger, A. \& Lenz, P. Are we ready for Autonomous Driving? The KITTI Vision Benchmark Suite. {\em Conference On Computer Vision And Pattern Recognition (CVPR)}. (2012)


\bibitem{kitti_2015}Menze, M. \& Geiger, A. Object Scene Flow for Autonomous Vehicles. {\em Conference On Computer Vision And Pattern Recognition (CVPR)}. (2015)


\bibitem{shift_2022}Sun, T. \& Segu, M. SHIFT: A Synthetic Driving Dataset for Continuous Multi-Task Domain Adaptation. {\em Computer Vision And Pattern Recognition}. (2022)


\bibitem{carla_2017}Dosovitskiy, A. \& Ros, G.  CARLA: An Open Urban Driving Simulator. {\em Proceedings Of The 1st Annual Conference On Robot Learning}. pp. 1-16 (2017)


\bibitem{citr}Yang, D. \& Ozguner, U. Top-view Trajectories: A Pedestrian Dataset of Vehicle-Crowd Interaction from Controlled Experiments and Crowded Campus.  (2019,6)


\bibitem{cityscapes_2016}Cordts, M. \& Omran, M. The Cityscapes Dataset for Semantic Urban Scene Understanding. {\em Proc. Of The IEEE Conference On Computer Vision And Pattern Recognition (CVPR)}. (2016)


\bibitem{bdd100k}Yu, F., Chen, H. \& Others. BDD100K: A Diverse Driving Dataset for Heterogeneous Multitask Learning. {\em CVPR} pp. 2633-2642 (2020)


\bibitem{once}Mao, J., Niu, M. \& Others One Million Scenes for Autonomous Driving: ONCE Dataset. {\em NeurIPS}. (2021)


\bibitem{atc}Brscic, D., Kanda, T., Ikeda, T. \& Miyashita, T. Person Tracking in Large Public Spaces Using 3-D Range Sensors. {\em Human-Machine Systems, IEEE Transactions On}. pp. 522-534 (2013)

\end{thebibliography}


